Topo-Geometrically Distinct Path Computation using Neighborhood-augmented Graph, and its Application to Path Planning for a Tethered Robot in 3D

Many robotics applications benefit from being able to compute multiple locally optimal paths in a given configuration space. Examples include path planning for of tethered robots with cable-length constraints, systems involving cables, multi-robot topological exploration & coverage, and, congestion reduction for mobile robots navigation without inter-robot coordination. Existing paradigm is to use topological path planning methods that can provide optimal paths from distinct topological classes available in the underlying configuration space. However, these methods usually require non-trivial and non-universal geometrical constructions, which are prohibitively complex or expensive in 3 or higher dimensional configuration spaces with complex topology. Furthermore, topological methods are unable to distinguish between locally optimal paths that belong to the same topological class but are distinct because of genus-zero obstacles in 3D or due to high-cost or high-curvature regions. In this paper we propose an universal and generalized approach to multiple, locally-optimal path planning using the concept of a novel neighborhood-augmented graph, search-based planning in which can compute paths that are topo-geometrically distinct. This approach can find desired number of locally optimal paths in a wider variety of configuration spaces without requiring any complex pre-processing or geometric constructions. Unlike the existing topological methods, resulting optimal paths are not restricted to distinct topological classes, thus making the algorithm applicable to many other problems where locally optimal and geometrically distinct paths are of interest. We demonstrate the use of our algorithm to planning for shortest traversible paths for a tethered robot in 3D with cable-length constraint, and validate the results in simulations and real robot experimentation.

==> pseudocodes/pseudo_LCS.tex <==

\begin{algorithm}
	\caption{Length Constrained Search (LCS)} \label{alg:LCS}
        \begin{algorithmic}[1]
        \Statex $G_{LCS}=$ \textit{lengthConstrainedSearch}($G_\mathcal{U},v_s,q_g$)
    \Statex \hrulefill
         \Statex Inputs: \begin{enumerate}[label=\alph*.]
         \item Neighborhood augmented graph $G_\mathcal{U}=(\mathcal{V}_\mathcal{U},E_\mathcal{U})$
         \item Start vertex $v_s = (q_s,\mathcal{U}_s) \in \mathcal{V}_\mathcal{U}$
        \item Goal coordinates $q_g=(x^1_g,\ldots,x^m_g) \in \mathcal{V}$
        \end{enumerate}
    \Statex Output: Graph $G_{LCS}$ \todo{Here happens another graph construction. However would that be counter-intuitive? Should it be some sort of a path reconstruction instead? (What we do is to generate another graph using the vertices and edges of the existing graph, but from a given start to a given goal. Then reconstruct the path using this graphs reconstruction method.)}
    \Statex \hrulefill
\State g-score: $g_{LCS}(v_s) := 0$
    \State Vertex set for LCS $\mathcal{V}_{LCS} = \{v_s\}$
    \State Edge set for LCS $E_{LCS} = \emptyset$
    \State Open list: $Q := \{v_s\}$
    \State $v:= v_s$
    % \While {$Q \neq \emptyset$ \textbf{AND} \textbf{not} \textit{areCoordsEqual}($v,q_g$)}
    \While {\textbf{not} \textit{stopSearchAtGoal}($Q,v,q_g$)}
        \State $v := arg\,min_{v' \in Q} g_{LCS}(v')$
        \State $Q = Q \setminus v$
        \State Successors: $S_{v} = \emptyset$
        \For {$v_i \in V_\mathcal{U}$, s.t. $\exists e \in E_\mathcal{U}$, with $e = (v,v_i)$}
            \State $g_{LCS}(v_i) = \infty$
            \If {$\nexists v_j \in \mathcal{V}_{LCS}$, with $v_i \equiv v_j$}
                \State $\mathcal{V}_{LCS} = \mathcal{V}_{LCS} \cup \{v_i\}$
                \State $E_{LCS} = E_{LCS} \cup \{(v,v_i)\}$
                \State $S_{v} = S_{v} \cup \{v_i\}$
            \Else
                \State $E_{LCS} = E_{LCS} \cup \{(v,v_j)\}$
                \State $S_{v} = S_{v} \cup \{v_j\}$
            \EndIf
            \EndFor
        \For {$v_k \in S_v$}
            \If {$v_k \notin Q$}
                \State $g_{LCS}' = g_{LCS}(v) + c(v,v_k)$
                \If {$g_{LCS}' < g_{LCS}(v_k)$}
                    \State $g_{LCS}(v_k) = g_{LCS}'$
                    \State $Q = Q \cup \{v_k\}$
                \EndIf
            \EndIf
        \EndFor
    \EndWhile
    \State $G_{LCS} := (\mathcal{V}_{LCS},E_{LCS})$
    \State \textbf{return} $G_{LCS}$
	\end{algorithmic} 
\end{algorithm}

==> pseudocodes/pseudo_basicAStar.tex <==

\begin{algorithm}
	\caption{Basic A*} \label{alg:basicAStar}
        \begin{algorithmic}[1]
         \Statex Inputs: \begin{enumerate}[label=\alph*.]
        \item Graph $G$ with vertex set $\mathcal{V}$
        \item Neighboring function $\mathcal{N}_G: V \to N_v \subset \mathcal{V}$
        \item Cost function $c(v_i,v_j): V \times V \to \mathbb{R}_+$
        \item Start node $v_0=(x_0,y_0,z_0) \in \mathcal{V}$
        \item Goal configuration $v_g=(x_g,y_g,z_g) \in \mathcal{V}$
        \end{enumerate}
    \Statex Output: An ordered set of vertices generating the shortest path from start to goal
    \Statex \hrulefill
    \State $g(v_i) := \infty$, $\forall v_i \in \mathcal{V}$
    \State $g(v_0) := 0$
    \State Open list: $Q := \{v_0\}$
    \While {$Q \neq \emptyset$ AND $v \neq v_g$}
        \State $v := arg\,min_{v' \in Q} g(v')$
        \State $Q = Q \setminus v$
        \For {$u \in \mathcal{N}_G(v)$}
            \If {$u \notin Q$}
                \State $g' = g(v) + c(v,u)$
                \If {$g' < g(u)$}
                    \State $g(u) = g'$
                    \State $Q = Q \cup \{u\}$
                \EndIf
            \EndIf
        \EndFor
    \EndWhile
    \State \textbf{return} path?
	\end{algorithmic} 
\end{algorithm}

\todo{Stopping criterion for Basic A* might be modified (represent with a function?)}

\todo{Define the check $u \notin Q$ via a function: How do we compare vertices?}

\todo{Path reconstruction, output, and return statements}

==> pseudocodes/pseudo_basicSearch.tex <==

\begin{algorithm}
	\caption{Search on Incrementally Constructed Graph} \label{alg:basicSearch}
        \begin{algorithmic}[1]
         \Statex Inputs: \begin{enumerate}[label=\alph*.]
         \item Start vertex $v_s = (x^1_s,\ldots,x^m_s) \in \mathcal{V}$
         \item Adjacency function $\mathcal{N}: v \to \mathcal{N}(v) \subset \mathcal{V}\times\ldots\times\mathcal{V}$
        \item Cost function $c(v_i,v_j): \mathcal{V} \times \mathcal{V} \to \mathbb{R}_+$
        \item Goal configuration $v_g=(x^1_g,\ldots,x^m_g) \in \mathcal{V}$
        \end{enumerate}
    \Statex Output: Graph $G$, with costs computed for every vertex
    \Statex \hrulefill
    \State g-score: $g(v_s) := 0$
    \State $\mathcal{V} = \{v_s\}$
    \State $E = \emptyset$
    \State Open list: $Q := \{v_s\}$
    \State $v:= v_s$
    \While {$Q \neq \emptyset$ \textbf{AND} $v \not\equiv v_g$}
        \State $v := arg\,min_{v' \in Q} g(v')$
        \State $Q = Q \setminus v$
        \State Successors: $S_{v} = \emptyset$
        \For {$v_i \in \mathcal{N}(v)$}
            \State $g(v_i) = \infty$
            \If {$\nexists v_j \in \mathcal{V}$, with $v_i \equiv v_j$} \Comment{Refer to $\equiv$}
                \State $\mathcal{V} = \mathcal{V} \cup \{v_i\}$
                \State $E = E \cup \{(v,v_i)\}$
                \State $S_{v} = S_{v} \cup \{v_i\}$
            \Else
                \State $E = E \cup \{(v,v_j)\}$
                \State $S_{v} = S_{v} \cup \{v_j\}$
            \EndIf
            \EndFor
        \For {$v_k \in S_v$}
            \If {$v_k \notin Q$}
                \State $g' = g(v) + c(v,v_k)$
                \If {$g' < g(v_k)$}
                    \State $g(v_k) = g'$
                    \State $Q = Q \cup \{v_k\}$
                \EndIf
            \EndIf
        \EndFor
    \EndWhile
    \State $G := (\mathcal{V},E)$
    \State \textbf{return} $G$
	\end{algorithmic} 
\end{algorithm}

==> pseudocodes/pseudo_mergePoints.tex <==

\begin{algorithm}
	\caption{Incremental Construction and Dijkstra's Search in a Neighborhood-augmented Graph (NAG) with Merge Points} \label{alg:mergePoints}
        \begin{algorithmic}[1]
        \Statex $G_\mathcal{U} =$ \textit{searchNAG\_MP}~($q_s,\mathcal{N}_G,\mathcal{C}_G, @\text{\textit{stopSearch}}$)
    \Statex \hrulefill
         \Statex Inputs:
         \begin{enumerate}[leftmargin=2em,label=\alph*.]
         \item Start configuration $q_s \in V$
         \item Neighbor/successor function $\mathcal{N}_G$ (this decsribes the connectivity of graph $G$)
        \item Cost function $\mathcal{C}_G: V \times V \to \mathbb{R}_+$
        \item Stopping criteria (function), \textit{stopSearch}: $V_\mathcal{U}\rightarrow \{0,1\}$
        \end{enumerate}
    \Statex Output: 
    \Statex \hspace{2em} Graph $G_\mathcal{U}$, with costs and neighborhoods computed for every vertex
    \Statex \hrulefill
    \State $v_s := (q_s,\{\& v_s\})$ \algcomment{start vertex in $V_\mathcal{U}$, with self-reference} 
    \Statex \phantom{$v_s := (q_s,\{\& v_s\})$} \algcomment{in its tangent neighborhood set.}
    \State Set $g(v_s) = 0$ \algcomment{g-score}
    \State $V_\mathcal{U} = \{v_s\}$ \algcomment{vertex set}
    \State $E_\mathcal{U} = \emptyset$ \algcomment{edge set, maintained implicitly as a link tree/graph}
    \State $Q = \{v_s\}$ \algcomment{open list, maintained by a heap data structure.}
    \State $v:= v_s$
    % \While {$Q \neq \emptyset$ \textbf{AND} \textbf{not} \textit{areCoordsEqual}($v,q_g$)}
    \While {$Q \neq \emptyset$ \textbf{AND} \textbf{not} \textit{stopSearch}($v$)}
        \State $v := (q,\mathcal{U}) = \arg\!\min_{v' \in Q} \, g(v')$ \algcomment{heap pop.}
        \State $Q = Q - v$ \algcomment{heap pop.}
        \If {$v .\text{is\_merge\_point}$}
        \State \textbf{continue}
        \EndIf
        \State $\mathcal{U}' =$ \textit{computeTNS}\,($v, G_\mathcal{U}$) \algcomment{tangent neighborhood set} \label{ln:computeTNS} 
        \Statex \phantom{$\mathcal{U}' =$ \textit{computeTNS}($G_\mathcal{U},v$)} ~~~~\algcomment{for path leading to $v$}
        \For {$q' \in \mathcal{N}_G(v)$}
            \State $v' := (q',\mathcal{U}')$ \algcomment{potential neighbor/successor}
            \State $g' = g(v) + \mathcal{C}_G(q,q')$ \algcomment{potential g-score for $v'$}
            \If {$\exists~ w \in V_\mathcal{U}$, with $v' \not\equiv w$ \textbf{AND} $q' = w.q$} 
                \Statex \phantom{.}\qquad\qquad \algcomment{new vertex at the same coordinates}
                \If{\textit{distanceInGraph}($v',w$) $ < \epsilon_{mp}$}
                \State $v'.\text{is\_merge\_point} = \textbf{True}$
                \State $w.\text{is\_merge\_point} = \textbf{True}$
                \EndIf
            \EndIf
            \If {$\nexists~ w \in V_\mathcal{U}$, with $v' \equiv w$} \algcomment{new vertex}
                \State $V_\mathcal{U} = V_\mathcal{U} \cup \{v'\}$
                \State $E_\mathcal{U} = E_\mathcal{U} \cup \{(v,v')\}$ \algcomment{maintained as linktree}
                \Statex \phantom{.}\qquad\qquad \algcomment{for neighbor function computation, $\mathcal{N}_{G_\mathcal{U}}$}
                \State $g(v') = g'$
                \State $Q = Q \cup \{v'\}$
                \State $v'.\text{came\_from} = v$
            \Else \algcomment{vertex already exists ($w$)}
                \State $E_\mathcal{U} = E_\mathcal{U} \cup \{(v,w)\}$
                \If {$g' < g(w)$ \textbf{AND} $w\in Q$} \algcomment{update $w$}
                    \State $g(w) = g'$
                    \State $w.\text{came\_from} = v$
                    \State $w =$ \textit{updateTNS}\,($w,v'$) \label{ln:update-tns}
                \EndIf
            \EndIf
            \EndFor
        % \For {$v_k \in S_v$}
        %     \If {$v_k \notin Q$}
        %         \State $g' = g(v) + c(v,v_k)$
        %         \If {$g' < g(v_k)$}
        %             \State $g(v_k) = g'$
        %             \State $Q = Q \cup \{v_k\}$
        %         \EndIf
        %     \EndIf
        % \EndFor
    \EndWhile
    \State $G_\mathcal{U} := (\mathcal{V}_\mathcal{U},E_\mathcal{U})$
    \State \textbf{return} $G_\mathcal{U}$
	\end{algorithmic} 
\end{algorithm}

==> pseudocodes/pseudo_stopSearchRadius.tex <==
\begin{algorithm}
	\caption{Radius-Based Stopping Criteria for Search} \label{alg:stopSearchRadius}
        \begin{algorithmic}[1]
        \Statex bool $=$ \textit{stopSearchAtRadius}($v$)
    \Statex \hrulefill
         \Statex Input: Current vertex $v = (q,\mathcal{U})$
        \Statex Static variable: Search depth/radius $r$
    \Statex Output: Boolean (\textbf{true} to stop search, \textbf{false} to continue)
    \Statex \hrulefill
    \If {$g(v) > r$}
        \State \textbf{return true}
    \Else
        \State \textbf{return false}
    \EndIf
	\end{algorithmic} 
\end{algorithm}

==> pseudocodes/pseudo_workspace_exploration.tex <==

\begin{algorithm}
	\caption{Workspace Exploration via Graph Construction} \label{alg:WSExploration}
        \begin{algorithmic}[1]
         \Statex Inputs: \begin{enumerate}[label=\alph*.]
         \item Base coordinates $q_b = (x^1_b,\ldots,x^m_b) \in \mathcal{V}$
         \item Adjacency function $\mathcal{N}: v \to \mathcal{N}(v) \subset \mathcal{V}\times\ldots\times\mathcal{V}$
        \item Cost function $c(v_i,v_j): \mathcal{V} \times \mathcal{V} \to \mathbb{R}_+$
        \item Maximum tether length $l$
        \end{enumerate}
    \Statex Output: Graph $G_\mathcal{U}$, with costs and neighborhoods computed for every vertex
    \Statex \hrulefill
    \State $v_s := (q_s,\mathcal{U}_s)$
    \State $\mathcal{U}_s := \{v_s\}$
    \State g-score: $g(v_s) := 0$
    \State $\mathcal{V}_\mathcal{U} = \{v_s\}$
    \State $E_\mathcal{U} = \emptyset$
    \State Open list: $Q := \{v_s\}$
    \State $v:= v_s$
    \While {$Q \neq \emptyset$ \textbf{AND} $g(v) < l$}
        \State $v := arg\,min_{v' \in Q} g(v')$
        \State $Q = Q \setminus v$
        \State Successors: $S_{v} = \emptyset$
        \For {$q_i \in \mathcal{N}(v)$}
            \State $\mathcal{U}_{q_i} =$ \textit{computeNeighborhood}($r,v$)
            \State $v_i := (q_i,\mathcal{U}_{q_i})$
            \State $g(v_i) = \infty$
            \If {$\nexists v_j \in \mathcal{V}_\mathcal{U}$, with $v_i \equiv v_j$}
                \State $\mathcal{V}_\mathcal{U} = \mathcal{V}_\mathcal{U} \cup \{v_i\}$
                \State $E_\mathcal{U} = E_\mathcal{U} \cup \{(v,v_i)\}$
                \State $S_{v} = S_{v} \cup \{v_i\}$
            \Else
                \State $E_\mathcal{U} = E_\mathcal{U} \cup \{(v,v_j)\}$
                \State $S_{v} = S_{v} \cup \{v_j\}$
            \EndIf
            \EndFor
        \For {$v_k \in S_v$}
            \If {$v_k \notin Q$}
                \State $g' = g(v) + c(v,v_k)$
                \If {$g' < g(v_k)$}
                    \State $g(v_k) = g'$
                    \State $Q = Q \cup \{v_k\}$
                \EndIf
            \EndIf
        \EndFor
    \EndWhile
    \State $G_\mathcal{U} := (\mathcal{V}_\mathcal{U},E_\mathcal{U})$
    \State \textbf{return} $G_\mathcal{U}$
	\end{algorithmic} 
\end{algorithm}

==> sections/literature_review.tex <==
\todo{Mostly Prof. Bhattacharya's papers on topological planning (h-augmented graph 2d and 3d). Geometry at large. Existing work on path planning for tethered robots?}

Focusing on the topological classification of the paths, several options have been explored on how to encode the topological information to be used when augmenting a graph. In this regard, \citep{Bhattacharya2012} leverages theorems from Complex Analysis and Electromagnetism to design differential 1-forms, whose integration along a path is homology invariant. The value of the integral is named as H-signature and it is used as the additional data to augment the graph with. Building up on this work, \citep{Bhattacharya2013} uses de Rham cohomology to design the differential 1-forms and hence the H-signature, expanding the approach to arbitrary dimensions and non-Euclidean spaces with punctures.

\cite{Bhattacharya2015a} proposes a differential 1-form corresponding to the angle spanned by a differential element, as an alternative representation to the one based on Complex Analysis introduced in \cite{Bhattacharya2012}. However by using $\mathbb{Z}_2$ coefficients, they obtain the H2-signature, a homology invariant that can detect winding around obstacles. A H2-Augmented Graph is then used for path planning in an environment with uncertainties.

A word-based homotopy invariant is described in \citep{Hatcher2001}. This description requires the construction of non-intersecting rays from the obstacles in the environment and the tracking of the number of times a path crosses each ray. As a simple representation in 2D environments with obstacles, the word-based homotopy invariant is used as the $h$-signature in \citep{Kim2014} to solve path planning problems for tethered robots and in \citep{Bhattacharya2015b} to manipulate objects using cables.

\citep{Bhattacharya2018} solves the word problem by leveraging Dehn's algorithm, extending the use of the word-based $h$-signature for knot/link complements in 3D Euclidean spaces and cylindrically deleted coordination space of multiple robots.
